Object-wise Masked Autoencoders for Fast Pre-training

Self-supervised pre-training for images without labels has recently achieved promising performance in image classification. The success of transformer-based methods, ViT and MAE, draws the community's attention to the design of backbone architecture and self-supervised task. In this work, we show that current masked image encoding models learn the underlying relationship between all objects in the whole scene, instead of a single object representation. Therefore, those methods bring a lot of compute time for self-supervised pre-training. To solve this issue, we introduce a novel object selection and division strategy to drop non-object patches for learning object-wise representations by selective reconstruction with interested region masks. We refer to this method ObjMAE. Extensive experiments on four commonly-used datasets demonstrate the effectiveness of our model in reducing the compute cost by 72% while achieving competitive performance. Furthermore, we investigate the inter-object and intra-object relationship and find that the latter is crucial for self-supervised pre-training.

==> SECTIONS/30_Method/algo.tex <==



\begin{algorithm}[t]
\caption{Pseudocode of ObjMAE in a PyTorch-like style.}
\label{alg:code}
\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{mm}: matrix multiplication; \texttt{cat}: concatenation.
%\vspace{-1.em}
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]
# f_e, f_d: encoder network and decoder network
# a: control the length of patches
# D: the hidden size of the encoder network

init(f_e.params,f_d.params) # initialize networks
for x,seg in loader:  # load a minibatch x with N samples
    seg = select(seg) # a segmentation mask of a random object on the image
    seq_x = patchfy(x)  # a sequence of image patches: Nx(H W)x(P P c)
    seq_seg = patchfy(seg)  # a sequence of segmentation patches: Nx(H W)

    # division process
    N, M, _ = seq_x.shape 
    num_patch = a * M
    seq_src, seq_tar = divide(seq_seg)  
    seq_src, seq_tar = align(seq_seg, num_patch)
    
    x_src = gather(seq_x, seq_src) # source patches: Nx(num_patch)x(P P c)
    x_tar = gather(seq_x, seq_src) # target patches: Nx(num_patch)x(P P c)
    
    # self-supervised task
    z_vis = f_e(x_src + gather(pos_embeds, seq_src)) # : Nx(num_patch)xD
    x_recon = f_d(cat(z_vis, mask_token + gather(pos_embeds, seq_tar))) #reconstructed patches: Nx(2 num_patch)xD
    loss = MSE(x_recon[-num_patch:], x_tar)

    # SGD update
    loss.backward()
    update(f_e.params)
    update(f_d.params)

\end{lstlisting}
\end{algorithm}

==> figs/obj_mask.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{pics/obj_mask.png}
    \caption{The object region of patches. }
    \label{fig:obj_mask}
\end{figure}

==> tabs/complexity.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
        \toprule
        Object Ratio & 1 & 0.5 &0.25 &0.125 \\
        \midrule
        MEAN (ms) & 268& 135&  74&  42 \\
        \midrule
        STD (ms) & 35& 13& 12&  6\\
        \bottomrule
    \end{tabular}
    \caption{Time consumption of ObjMAE on TITAN RTX (batch size is 256).}
    \label{tab:complexity}
\end{table}
